Responsive Parallelism with Synchronization

Many concurrent programs assign priorities to threads to improve responsiveness. When used in conjunction with synchronization mechanisms such as mutexes and condition variables, however, priorities can lead to priority inversions, in which high-priority threads are delayed by low-priority ones. Priority inversions in the use of mutexes are easily handled using dynamic techniques such as priority inheritance, but priority inversions in the use of condition variables are not well-studied and dynamic techniques are not suitable. In this work, we use a combination of static and dynamic techniques to prevent priority inversion in code that uses mutexes and condition variables. A type system ensures that condition variables are used safely, even while dynamic techniques change thread priorities at runtime to eliminate priority inversions in the use of mutexes. We prove the soundness of our system, using a model of priority inversions based on cost models for parallel programs. To show that the type system is practical to implement, we encode it within the type systems of Rust and C++, and show that the restrictions are not overly burdensome by writing sizeable case studies using these encodings, including porting the Memcached object server to use our C++ implementation.

==> Makefile <==
PDFLATEX = pdflatex -file-line-error -halt-on-error
LATEX = latex

#default: pstopdf
default: pdf


abstract.txt: abstract.tex
	./pull-abstract

# pldi229-chenappendix.zip : pldi229-chenappendix.pdf
#	cp -a pldi229-chenappendix.pdf pldi229-chenappendix/
#	rm pldi229-chenappendix.zip 2> /dev/null || true
#	zip -r pldi229-chenappendix.zip pldi229-chenappendix -i \*.txt \*.pdf

bib: 
	$(PDFLATEX) main 
	bibtex main || true
	bibtex new || true
	bibtex thisbib || true
	$(PDFLATEX) main 

dvi: 
	$(LATEX) main

ps: dvi
	dvips -P pdf -o main.ps -t letter main

pstopdf: ps
	ps2pdf -dPDFSETTINGS=/printer -dEmbedAllFonts=true main.ps main.pdf

pdf: bib 
	$(PDFLATEX) main

final: clean bib

clean: 
	rm -f *.aux main.dvi main.bbl main.blg *.log *.out main.brf main.ps main.pdf pldi229-chen.pdf pldi229-chenappendix.pdf

impl-tar:
	tar -cvzf type-system-implementations.tgz rust/ cpp/


==> email_case_study.tex <==
\subsection{C++ Case Study I: Memcached}

We have ported the Memcached object caching server~\cite{Memcached09} (v1.5.13)
to utilize our C++ type system.  The Memcached server acts as a distributed
in-memory cache. It is a key-value store, with the core purpose of maintaining a
hash table of objects that can be updated or retrieved by clients.  Memcached is
written in C, and uses pthreads and I/O multiplexing in order to handle many
clients.   

The Memcached itself consists of multiple long-running threads (i.e., tasks).
The main thread performs most of the setup code and spawns off other
long-running threads, such as a resize thread that performs hashtable resizing
when necessary, a LRU maintenance thread that maintains the (approximately)
least-recently-used (LRU) ordering of items in buckets in the hash table, a LRU
crawler thread that frees up items that have gone ``cold'' in the cache, a slab
maintainer thread for balancing free memory between different size classes of
Memcached's internal memory pool, and a logger thread that crawls the hashtable
to collect statistics about items in the cache.

Overall, we wrote the applications with three different priority levels ---
whenever the actual resizing occurs, it is done as a high-priority task (spawned
off by the resizing thread); on the other hand, any logging related activities
are done as low-priority tasks.  Things relating to handling the client request,
maintaining LRUs of the cache, and memory pool management are done as 
medium-priority tasks.

Three different conditional variables are used in the code.  Currently, all the
signaling and waiting happen to be done within medium priority tasks, which
works out well, as the signaling and waiting on CVs all happen within critical
sections surrounded by lock-acquire and lock-release operations.\footnote{As
explained in \secref{overview}, threads acquiring the same lock must have the
same priority level to avoid priority inversions.}  

Today, we could have had more fine-grained priority levels among the threads
that are currenlty in medium priority.  Doing so would have require us to lift
some of the critical sections into its own tasks an potentially promote CVs from
lower to higher priorities at more places, but we could have still made the
types work out so that the whole application type checks.  We chose not to have
more fine-grained priority levels, as all the tasks currently running at the
same medium priority level are inter-dependent (e.g., client request may run out
of memory if the slab thread runs at a lower priority or if the LRU crawler
thread does not free the memory in time).


\subsection{C++ Case Study: Email Client}

We implemented a multi-user shared email server based on the version released
by prior work~\citep{MullerSiGoAcAgLe20} to demonstrate the expressiveness of
our C++ implementation.  The server utilizes 5 priority levels.  At the
highest priority, the server accepts new client connections (one thread per
connection), listen to requests from connected clients, and spawns off other
types of threads to perform requests received: \code{send} threads process
requests to send emails (highest priority); \code{sort} threads handle
requests for sorting emails (2nd highest); and \code{compress} threads
compress emails and \code{print} threads handle requests to print emails (3rd
highest).  There is also a \code{dequeue} thread that dequeues compression
tasks that arise from sending emails and generates threads to perform the
compressions (4th highest).  The main thread, which performs setup and
teardown tasks, is at the lowest priority.

The interesting interaction is how \code{compress} threads are generated.  Two
different kinds of threads interact in a multi-producer/single consumer model:
the (multiple) \code{send} threads act as producers, and the \code{dequeue}
thread acts as the consumer.  Since the number of \code{send} threads is not
known at compile time (depends on the number of send requests), we utilizes
the alternative splitting macro (that does not invalidate the input) within a
loop to split off CV signal permissions as we spawn off each \code{send}
thread.
%
When a \code{send} thread pushes the number of emails in an inbox over a
threshold of uncompressed messages, it enqueues information on what to
compress and signals the \code{dequeue} thread to wake up and generate a
\code{compress} thread.
%
The email system consists of 1250 lines of code. XXX Kyle is this still accurate?


%Initially all emails arrive and are stored uncompressed. As
%\texttt{send} threads execute, they check the recipient's inbox size to
%determine if there is enough uncompressed data to trigger a compression. If so,
%they take a global lock with a priority ceiling of \texttt{HighP},
%\texttt{compress\_lock}, enqueue a compression task in a global queue,
%\texttt{compress\_q}, and signal a condition variable, \texttt{compress\_cv},
%that was passed into the \texttt{send} thread via spawn. The \texttt{dequeue}
%thread, meanwhile, loops on locking \texttt{compress\_lock}, checking
%\texttt{compress\_q}, and if the queue is empty waiting on a reference to the
%same \texttt{compress\_cv}. If the queue was not empty, then the
%\texttt{dequeue} thread empties the queue, exits the critical section, and
%generates compression threads for each compress task.  The \texttt{compress\_cv}
%is passed to the necessary threads in much the same was as shown in
%\figref{pc-fixed}. Initially, \texttt{compress\_cv} has priority \texttt{LowP}.
%After passing ownership along for signaling, it is promoted to \texttt{HighP}
%and passed to the \texttt{dequeue} thread as a non-owning
%reference.

%\punt{
%\begin{figure}
%\begin{lstlisting}
%cilk::mutex compress_lock; // global lock
%std::queue<compress_task_t> compress_task_queue; // global queue
%...
%int main<LowPrio>(int argc, char *argv[]) {
%    ...
%    cilk_decl_cond_var(compress_cv, LowPrio);
%    cilk_split_cond_var_ownership(compress_cv,
%        signal_cv,
%        (std::array{none, shared, shared, shared, shared}), // signal_cv ownership
%        wait_cv); // wait_cv ownership is deduced from signal_cv ownership
%    cilk_pspawn(HighestPrio, acceptConnections,
%        cilk_func_call_transfer_ownership(signal_cv));
%    cilk_cond_var_promote(wait_cv, promoted_cv, DequeuePrio);
%    cilk_cond_var_get_ref(promoted_cv, promoted_cv_ref);
%    cilk_pspawn(DequeuePrio, dequeueCompression, cilk_func_call_copy_ref(promoted_cv_ref));
%    ...
%}
%\end{lstlisting}
%\caption{Setup necessary to signal and wait on the compression task queue's
%condition variable.}
%\end{figure}
%}


